Detection and Combining Techniques for Asynchronous Random Access with Time Diversity

Asynchronous random access (RA) protocols are particularly attractive for their simplicity and avoidance of tight synchronization requirements. Recent enhancements have shown that the use of successive interference cancellation (SIC) can largely boost the performance of these schemes. A further step forward in the performance can be attained when diversity combining techniques are applied. In order to enable combining, the detection and association of the packets to their transmitters has to be done prior to decoding. We present a solution to this problem, that articulates into two phases. Non-coherent soft-correlation as well as interference-aware soft-correlation are used for packet detection. We evaluate the detection capabilities of both solutions via numerical simulations. We also evaluate numerically the spectral efficiency achieved by the proposed approach, highlighting its benefits.

==> sections/how_it_works.tex <==
\section{How it works}

The system should work like this:
\begin{itemize}
\item Detection of possible replicas done in two phases
\begin{enumerate}
\item In the first phase we correlate over the entire received frame looking for the sync. word. We use a threshold for determining possible replicas positions.
\item For all candidates, we take the received signal corresponding to one packet duration after the candidate peak and we correlate this signal with all other peaks identified in phase 1 (except for the peaks that are less than one packet duration away from the identified peak).
\end{enumerate}
\item After this procedure we have all candidates replicas and the corresponding correlation values. We order the correlation results in descending order. We pick the first $d$-1 location and we assume that these are the replicas corresponding to the same user.
\item If the coupling of candidates is correct, we increase by 1 the number of correctly coupled replicas of users.
\end{itemize}

When we introduce discretization in the location of replicas user by user, the procedure is like this instead:
\begin{itemize}
\item Detection of possible replicas done in two phases
\begin{enumerate}
\item In the first phase we correlate over the entire received frame looking for the sync. word. We use a threshold for determining possible replicas positions.
\item For all candidates, we take the received signal corresponding to one packet duration after the candidate peak and we correlate this signal with all peaks identified in phase 1 that fulfill the following constraints
\begin{enumerate}
\item Are within an interval in the discretized position of the current user.
\item Are at least one packet away from the current peak candidate.
\end{enumerate}
\end{enumerate}
\item After this procedure we have all candidates replicas and the corresponding correlation values. We order the correlation results in descending order. We pick the first $d$-1 location and we assume that these are the replicas corresponding to the same user.
\item If the coupling of candidates is correct, we increase by 1 the number of correctly coupled replicas of users.
\end{itemize}

\section{Old Stuff}

We start looking at one packet duration $T_p$ before the possible start of the synchronization word, which corresponds to the \emph{vulnerable period} i.e. the interval of time in which any packet arrival will cause a collision with the synchronization word. We assume that the snyc word duration $T_{sw}$ is much shorter than a packet duration, i.e. $T_{sw}<<T_p$. Thanks to this we will not consider border effects, i.e. all collisions are involving the full sync word.

At the transmitter side, the $k$-th interference signal $s_k(t)$ will be
\[
s_k(t)=\sum_{i=1}^{n}a_i^{(k)}g(t-iT_s),
\]
where $n$ is the number of symbols composing the packet, $\left\{a_i^{(k)}\right\}$ is the symbols sequence and $T_s$ is the symbol period. The signal $r_k(t)$ seen at the receiver after the \ac{MF} corresponding to the $k$-th interference is
\[
r_k(t)\cong s_k(t-lT_s-\epsilon_k)e^{j\left(2\pi f_k t + \varphi_k\right)},
\]
with a random delay $\epsilon_k \sim \mathcal{U}\left[0;T_s\right)$, a random frequency offset $f_k \sim \mathcal{U}\left[-f_{max};f_{max}\right]$ and a random phase offset $\varphi_k\sim \mathcal{U}\left[0;2\pi\right)$. The approximation of the received signal holds tight if $f_{max}T_s<<1$. The overall interference is the summation over all interferers of $r_k(t)$ which can be explicitly written as in equation \eqref{eq:int_1}.
\begin{figure*}[!t]
\begin{equation}
\setcounter{equation}{1}
\sum_k r_k(t)=\sum_{z=-n}^{n_{sw}} \sum_{w_z=1}^{N_z} \sum_{\mu=1}^{n} a_\mu^{(z,w_z)}g(t-\mu T_s-z T_s - \epsilon_{z,w_z}) e^{j2\pi\left(f_{z,w_z} t+\varphi_{z,w_z}\right)}.
\label{eq:int_1}
\end{equation}
\end{figure*}
The first summation is over all the considered symbols (from $n$ symbols before the sync word to the end of it), while the second is over the total of interferers starting in symbol $z$, univocally identifying the interferer packet. The last summation is over all symbols of the packet. In this way, the received signal $y(t)$ can be written as
\[
y(t)=x(t)+\sum_k r_k(t)+n(t),
\]
where $n(t)\sim \mathcal{CN}(0,\sigma_n^2)$ is the \ac{AWGN} and $x(t)$ represents the synchronization word signal. After sampling at the Nyquist rate $kT_s$ the received signal $y_h$ can be written as in equation \eqref{eq:rx_1}.
\begin{figure*}[!t]
\begin{equation}
\setcounter{equation}{2}
y_h=x_h+\sum_{w_z=1}^{N_z} \sum_{\mu=1}^{n} a_\mu^{(h,w_h)}g(T_s(k-\mu-h) - \epsilon_{h,w_h}) e^{j2\pi\left(f_{h,w_h} k T_s+\varphi_{h,w_h}\right)} + n_h
\label{eq:rx_1}
\end{equation}
\end{figure*}
Assuming Gaussian codebooks, $a_\mu^{(z,w_z)}\sim \mathcal{CN}(0,P_I)$. In this way we have
\[
y_h=x_h+\nu_h+n_h,
\]
where $\nu_h \sim \mathcal{CN}(0,N_I\cdot P_I)$ is a complex Gaussian random variable. $N_I$ is itself a random variable that represents the number of interferers at time instant $hT_s$, in this way $N_I\sim \mathcal{P}oiss\left( G\cdot\frac{T_p+T_{sw}}{T_p}\right)$ is Poisson distributed.

We now focus on the possible location of the synchronization word. Along this $n_{sw}$ symbols, from statistical theory of hypothesis testing we have
\[
\begin{aligned}
\mathcal{H}_0&:r_h=\nu_h+n_h\quad\quad\quad\text{for}\quad h=1,...,n_{sw}\\
\mathcal{H}_1&:r_h=c_h+\nu_h+n_h\quad\text{for}\quad h=1,...,n_{sw}
\end{aligned}
\]
Using the notation $\mathbf{R}=(R_1,...,R_{n_{sw}})$ for the r.v. corresponding to the vector $\mathbf{r}=(r_1,...,r_{n_{sw}})$ of the received samples, the likelihood ratio test is
\[
\Lambda(\mathbf{r})= \frac{f_{\mathbf{R}|\mathcal{H}_1}(\mathbf{r}|\mathcal{H}_1)} {f_{\mathbf{R}|\mathcal{H}_0}(\mathbf{r}|\mathcal{H}_0)} \underset{\mathcal{D}_1}{\overset{\mathcal{D}_0}{\gtrless}} \lambda
\]
where $f_{\mathbf{R}|\mathcal{H}_l}$ is the \ac{PDF} of $\mathbf{R}$ under the hypotheses $\mathcal{H}_l,l\in \left\{0,1\right\}$, and $\lambda$ is the selected threshold. According to the test, $\Lambda(\mathbf{r})>\lambda$ corresponds to the decision $\mathcal{D}_1$, i.e. we decide we are in the presence of a sync word; otherwise the decision is $\mathcal{D}_0$. Since the channel and the interference are memoryless we also have
\[
f_{\mathbf{R}|\mathcal{H}_l}(\mathbf{r}|\mathcal{H}_l) = \prod_{h=1}^{n_{sw}} f_{R_h|\mathcal{H}_l}(r_h|\mathcal{H}_l)
\]
Given $\mathcal{H}_1$, the $R_h$ are a infinite sum of weighted Gaussian r.v.s., due to the interferers, plus a Gaussian with variance $\sigma_n^2$ and mean $c_h$, i.e.,
\begin{equation}
\begin{aligned}
f_{R_h|\mathcal{H}_1}(r_h|\mathcal{H}_1) &= \frac{1}{\sqrt{2\pi \sigma_n^2}} e^{-\frac{(r_h-c_h)^2}{2\sigma_n^2}} +\\
&+ \left[ \sum_{u=1}^{\infty} \frac{e^{-G'}G^{'u}}{u!} \left( \frac{1}{\sqrt{2\pi u P_I}} e^{-\frac{(r_h-c_h)^2}{2u P_I}}\right)\right].
\end{aligned}
\end{equation}
Under the hypothesis $\mathcal{H}_0$ instead we have
\begin{equation}
\begin{aligned}
f_{R_h|\mathcal{H}_0}(r_h|\mathcal{H}_0) &= \frac{1}{\sqrt{2\pi \sigma_n^2}} e^{-\frac{r_h^2}{2\sigma_n^2}} +\\
&+ \left[ \sum_{u=1}^{\infty} \frac{e^{-G'}G^{'u}}{u!} \left( \frac{1}{\sqrt{2\pi u P_I}} e^{-\frac{r_h^2}{2u P_I}}\right)\right].
\end{aligned}
\end{equation} 


==> tex/displaynotation.tex <==

\cleardoublepage

\section*{Notation}


\bigskip

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\load$ & \verb;\load; & Load \\
$\thrp$ & \verb;\thrp; & Throughput \\
$\thr$ & \verb;\thr; & Threshold \\
$\plr$ & \verb;\plr; & Packet loss probability \\
$\plrt$ & \verb;\plrt; & Packet loss probability target\\
${\ET}$ &  \verb;\ET; & Energy per transmission \\
${\EL}$ & \verb;\EL; & Energy cost of listening in one slot \\
${\EI}$ & \verb;\EI; & Energy cost of being idle in one slot \\
${\E}$ & \verb;\E; & Average energy spend per slot \\
${\La}$ &  \verb;\La; & Node-perspective UN dd \\
${\Rh}$ & \verb;\Rh; & Node-perspective SN dd \\
${\la}$ & \verb;\la; & Edge-perspective UN dd \\
${\rh}$ & \verb;\rh; & Edge-perspective SN dd \\
${\iLa{i}}$ & \verb;\iLa{i}; & Node-perspective UN dd seen by user $i$ \\
${\iRh{i}}$ & \verb;\iRh{i}; & Node-perspective SN dd seen by user $i$ \\
${\ila{i}}$ &\verb;\ila{i}; & Edge-perspective UN dd seen by user $i$ \\
${\irh{i}}$ &\verb;\irh{i}; & Edge-perspective SN dd seen by user $i$ \\
$\dum$  &\verb;\dum; & Dummy variable for dd polynomials, $\la(\dum)$  \\
$\graph$  &\verb;\graph; & Bipartite graph  \\
$\uset$  &\verb;\uset; & User nodes set  \\
$\sset$  &\verb;\sset; & Slot nodes set  \\
$\slots$ & \verb;\slots; & number of slots per discovery phase \\
$\users$ & \verb;\users; & number of users in the network \\
$\degree$ & \verb;\degree; & number of replicas sent per user, i.e. degree \\
$\avgd$ & \verb;\avgd; & average number of replicas sent per user, i.e. average degree \\
$\listn$ & \verb;\listn; & fraction of slots in listening over the total number of slots in a frame\\
$\dcost$ & \verb;\dcost; & Discovery cost\\
\hline \hline
\end{tabular}
\end{center}




\begin{center}
\begin{tabular}{ l l l}
\hline \hline
\hline \hline
\end{tabular}
\end{center}











\clearpage 

==> tex/notation.tex <==
\newtheorem{thm}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{coroll}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{result}{Result}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}


\newcommand{\ul}{ul}
\newcommand{\dl}{dl}
\newcommand{\load}{\mathsf{G}}
\newcommand{\tp}{\mathsf{S}}
\newcommand{\tpSA}{\tp_{sa}}
\newcommand{\tpUL}{\tp_{\ul}}
\newcommand{\tpULk}[1]{\tp_{\ul,#1}}
\newcommand{\tpDL}{\tp_{\dl}}
\newcommand{\dlrate}{\mathsf{R}}
\newcommand{\dlratek}{\mathsf{R}_k}
\newcommand{\fracratek}{z_k}
\newcommand{\plos}{\xi}
\newcommand{\x}{\mathtt{x}}
\newcommand{\qtarget}{\bar{\mathtt{q}}}
\newcommand{\plostarget}{\bar{\plos}}
\newcommand{\nrx}{K}
\newcommand{\usersRV}{U}
\newcommand{\users}{u}
\newcommand{\collRV}{C}
\newcommand{\coll}{c}
\newcommand{\peras}{\varepsilon}
\newcommand{\capDL}{\mathsf{C_{\dl}}}
\newcommand{\ulslot}{\mathsf{T_{\ul}}}
\newcommand{\dlslot}{\mathsf{T_{\dl}}}
\newcommand{\numulslot}{M_{\ul}}
\newcommand{\numdlslot}{M_{\dl}}
\newcommand{\slot}{m}
\newcommand{\del}{\mathsf{D}}
\newcommand{\maxdel}{\mathsf{D}_{max}}
\newcommand{\nsym}{n}
\newcommand{\bufsize}{B}



\newcommand{\oleq}[1]{\overset{\text{(#1)}}{\leq}}
\newcommand{\oeq}[1]{\overset{\text{(#1)}}{=}}
\newcommand{\ogeq}[1]{\overset{\text{(#1)}}{\geq}}
\newcommand{\ogeql}[2]{\overset{#1}{\underset{#2}{\gtreqless}}}










%%%%% Color for Editorial Changes
\definecolor{gl}{rgb}{0.0,0.5,0.8}
\definecolor{fc}{rgb}{0.8,0.5,0}
\definecolor{al}{rgb}{1,0.3,0.3}
\newcommand{\giangio}{\textcolor{gl}}
\newcommand{\fede}{\textcolor{fc}}
\newcommand{\alert}{\textcolor{al}}








==> tools/README <==

December 27, 2012


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class, specifically the section covering IEEE-style
lists and the Appendix covering the IEEEeqnarray commands.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later

 3. the IEEE itemize, enumerate and description list environments

 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 5. The IEEEproof environment.
 
 6. \IEEEauthorrefmark{}

IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
12/2012 V1.3 (V1.8 of IEEEtran.cls) changes:

 1) No longer redefines the standard LaTeX itemize, enumerate and 
    description (IED) lists by default. (e.g., the older package option
    "retainorgcmds" is now the default behavior.) A new package option,
    "redeflists", can be invoked to redefine the standard IED list
    environments to their IEEE versions. IEEEitemize, IEEEenumerate and
    IEEEdescription remain available in any case. The redeflists option
    may not be compatible with other packages that alter the standard
    IED list environments.

 2) Added new *-forms of \IEEEyesnumber*, \IEEEnonumber*, \IEEEyessubnumber*,
    and \IEEEnosubnumber* (the non-star form of the latter is also new) which
    persist across IEEEeqnarray lines until countermanded. To provide for
    continued subequations across instances of IEEEeqnarrays as well as for
    subequations that follow a main equation (e.g., 14, 14a, 14b ...)
    \IEEEyessubnumber no longer automatically increments the equation number
    on it's first invocation of a subequation group. Invoke both
    \IEEEyesnumber\IEEEyessubnumber together to start a new
    equation/subequation group.

 3) Hyperref links now work with IEEEeqnarray equations.
    Thanks to Stefan M. Moser for reporting this problem.

 4) Now provides the IEEEproof environment, as well as the
    \IEEEQEDhere, \IEEEQEDhereeqn and \IEEEQEDoff commands.
    Also, \IEEEproofindentspace allows users to change the
    IEEEproof indentation via \renewcommand.
    Thanks to Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser
    for suggesting this. Special thanks to Stefan M. Moser for beta
    testing and additional suggestions which improved IEEEproof.

 5) Revised \IEEEeqnarraymulticol{} to allow inner alignments without
    requiring extra containing braces to prevent an incomplete \ifx error.
    Thanks to Stefan M. Moser and Auke van der Valk for reporting this
    problem.

 6) Added \IEEEauthorrefmark.

 7) Removed support for legacy IED list commands.
    IEEEtrantools no longer defines or references \labelindent so as to
    avoid namespace problems with list packages that define it.
    Thanks to Sven Köhler for reporting the problem with enumitem.sty.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

changelog.txt         - The complete changelog history.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt, changelog.txt
***************************************************************************


